Linking of Lagrangian Tori and Embedding Obstructions in Symplectic 4-Manifolds

We classify weakly exact, rational Lagrangian tori in $T^* \mathbb{T}^2- 0_{\mathbb{T}^2}$ up to Hamiltonian isotopy. This result is related to the classification theory of closed $1$-forms on $\mathbb{T}^n$ and also has applications to symplectic topology. As a first corollary, we strengthen a result due independently to Eliashberg-Polterovich and to Giroux describing Lagrangian tori in $T^* \mathbb{T}^2-0_{\mathbb{T}^2}$ which are homologous to the zero section. As a second corollary, we exhibit pairs of disjoint totally real tori $K_1, K_2 \subset T^*\mathbb{T}^2$, each of which is isotopic through totally real tori to the zero section, but such that the union $K_1 \cup K_2$ is not even smoothly isotopic to a Lagrangian. In the second part of the paper, we study linking of Lagrangian tori in $(\mathbb{R}^4, \omega)$ and in rational symplectic $4$-manifolds. We prove that the linking properties of such tori are determined by purely algebro-topological data, which can often be deduced from enumerative disk counts in the monotone case. We also use this result to describe certain Lagrangian embedding obstructions.

==> linking_tori_4manifolds_bibliography.tex <==
%\documentclass{article}
%\usepackage{amssymb}
%\usepackage{amsmath}
%\usepackage{amsrefs}
%\usepackage[colorlinks=true]{hyperref}
%\usepackage{hyperref}
%\usepackage{cleveref}
%\usepackage{setspace}
%\usepackage{amscd}
%\usepackage{amsthm}
%\usepackage{mathtools}
%\usepackage{amsrefs}

%\begin{document}
%\begin{bibdiv}
%\begin{biblist}*{labels={alphabetic}}


\bib{abbas-hofer}{book}{
   author={Abbas, Casim},
   author={Hofer, Helmut},
   title={Holomorphic curves and global questions in contact geometry},
   series={Birkh\"{a}user Advanced Texts: Basler Lehrb\"{u}cher. [Birkh\"{a}user
   Advanced Texts: Basel Textbooks]},
   publisher={Birkh\"{a}user/Springer, Cham},
   date={2019},
   pages={xii+322},
   isbn={978-3-030-11802-0}
}

\bib{abouzaid-kragh}{article}{
   author={Abouzaid, Mohammed},
   author={Kragh, Thomas},
   title={Simple homotopy equivalence of nearby Lagrangians},
   journal={Acta Math.},
   volume={220},
   date={2018},
   number={2},
   pages={207--237}
}

\bib{abou-man}{article}{
title={A sheaf-theoretic model for $\operatorname{SL}(2,\mathbb{C})$ Floer homology},
author={Abouzaid, Mohammed},
author={Manolescu, Ciprian},
   journal={J. Eur. Math. Soc. (JEMS)},
   status={to appear.},
}

\bib{auroux}{article}{
title={Infinitely many monotone Lagrangian tori in $\mathbb{R}^6$}
author={Auroux, Denis}
journal={Invent. Math.}
volume={201}
number={3}
date={2016}
pages={909--924}}

\bib{banyaga}{article}{
   author={Banyaga, Augustin},
   title={Sur la structure du groupe des diff\'{e}omorphismes qui pr\'{e}servent une
   forme symplectique},
   language={French},
   journal={Comment. Math. Helv.},
   volume={53},
   date={1978},
   number={2},
   pages={174--227}
}

\bib{borrelli}{article}{
title={New examples of Lagrangian rigidity}
author={Borrelli, Vincent}
journal={Israel J. Math.}
volume={125}
date={2001}
pages={221--235}}


\bib{sftcompactness}{article}{
title={Compactness results in symplectic field theory}
author={Bourgeois, Fr\'{e}d\'{e}ric}
author={Eliashberg, Yakov}
author={Hofer, Helmut}
author={Wysocki, Krzysztof}
author={Zehnder, Eduard}
journal={Geom. Topol.}
volume={7}
date={2003}
pages={799--888}}



\bib{charette}{article}{
   author={Charette, Fran\c{c}ois},
   title={A geometric refinement of a theorem of Chekanov},
   journal={J. Symplectic Geom.},
   volume={10},
   date={2012},
   number={3},
   pages={475--491}
}
		
\bib{charette1}{article}{
   author={Charette, Fran\c{c}ois},
   title={Gromov width and uniruling for orientable Lagrangian surfaces},
   journal={Algebr. Geom. Topol.},
   volume={15},
   date={2015},
   number={3},
   pages={1439--1451}
}		


\bib{chekanov}{article}{
title={Lagrangian intersections, symplectic energy, and areas of holomorphic curves}
author={Chekanov, Yuri}
journal={Duke Math. J.}
volume={95}
number={1}
date={1998}
pages={213--226}}


\bib{chek-schlenk}{article}{
title={Lagrangian product tori in tame symplectic manifolds}
author={Chekanov, Yuri}
author={Schlenk, Felix}
journal={Comment. Math. Helv.}
volume={91}
number={3}
date={2016}
pages={445--475}}


\bib{cho}{article}{
title={Holomorphic discs, spin structures, and Floer cohomology of the Clifford torus}
author={Cho, Cheol-Hyun}
journal={Int. Math. Res. Not.}
number={35}
date={2004}
pages={1808--1848}}


\bib{cieliebak-eliashberg}{book}{
   author={Cieliebak, Kai},
   author={Eliashberg, Yakov},
   title={From Stein to Weinstein and back},
   series={American Mathematical Society Colloquium Publications},
   volume={59},
   note={Symplectic geometry of affine complex manifolds},
   publisher={American Mathematical Society, Providence, RI},
   date={2012},
   pages={xii+364}
}

\bib{cmsftcompactness}{article}{
title={Compactness for punctured holomorphic curves}
author={Cieliebak, Kai}
author={Mohnke, Klaus}
journal={ J. Symplectic Geom.}
volume={3}
number={4}
date={2005}
pages={589--654}}


\bib{cmaudin}{article}{
title={Punctured holomorphic curves and Lagrangian embeddings}
author={Cieliebak, Kai}
author={Mohnke, Klaus}
journal={Invent. Math.}
volume={212}
number={1}
date={2018}
pages={213--295}}


\bib{cooper-long}{article}{
   author={Cooper, Daryl},
   author={Long, Darren},
   title={Remarks on the $A$-polynomial of a knot},
   journal={J. Knot Theory Ramifications},
   volume={5},
   date={1996},
   number={5},
   pages={609--628}
}

\bib{cote}{article}{
author = {C\^{o}t\'{e}, Laurent}
title = {On Linking of Lagrangian Tori in $\mathbb{R}^4$}
journal= {J. Symplectic Geom.}
%eprint = {1806.07853}
year = {2018}
status={To appear}
}



\bib{damian}{article}{
title={Floer homology on the universal cover, a proof of Audin's conjecture and other constraints on Lagrangian submanifolds.}
author={Damian, Mihai}
journal={Comment. Math. Helv.}
volume={87}
date={2012}
pages={433--463}}


\bib{dim1}{article}{
author = {Dimitroglou Rizell, Georgios}
title = {The classification of {L}agrangians nearby the {W}hitney immersion}
journal={Geom. Topol.}
status={To appear}
%eprint = {1712.01182}
year = {2017}}

\bib{dim-evans}{article}{
title={Unlinking and unknottedness of monotone Lagrangian submanifolds}
author={Dimitroglou Rizell, Georgios}
author={Evans, Jonathan David}
journal={Geom. Topol.}
volume={18}
number={2}
date={2014}
pages={997--1034}}

\bib{dgi}{article}{
title={Lagrangian isotopy of tori in $S^2 \times S^2$ and $\mathbb{CP}^2$}
author={Dimitroglou Rizell, Georgios}
author={Goodman, Elizabeth}
author={Ivrii, Alexander}
journal={Geom. Funct. Anal.}
volume={26}
number={5}
date={2016}
pages={1297--1358}}




\bib{ekholm-smith}{article}{
   author={Ekholm, Tobias},
   author={Smith, Ivan},
   title={Nearby Lagrangian fibers and Whitney sphere links},
   journal={Compos. Math.},
   volume={154},
   date={2018},
   number={4},
   pages={685--718}
}



\bib{eliash}{article}{
   author={Eliashberg, Yakov},
   title={Topology of $2$-knots in $\mathbb{R}^4$ and symplectic geometry},
   conference={
      title={The Floer memorial volume},
   },
   book={
      series={Progr. Math.},
      volume={133},
      publisher={Birkh\"auser, Basel},
   },
   date={1995},
   pages={335--353}}

\bib{sft}{article}{
   author={Eliashberg, Yakov},
   author={Givental, Alexander},
   author={Hofer, Helmut},
   title={Introduction to symplectic field theory},
   note={GAFA 2000 (Tel Aviv, 1999)},
   journal={Geom. Funct. Anal.},
   date={2000},
   number={Special Volume},
   pages={560--673}
}

\bib{eli-pol}{article}{
   author={Eliashberg, Yakov},
   author={Polterovich, Leonid},
   title={New applications of Luttinger's surgery},
   journal={Comment. Math. Helv.},
   volume={69},
   date={1994},
   number={4},
   pages={512--522}}

\bib{eli-pol2}{article}{
   author={Eliashberg, Yakov},
   author={Polterovich, Leonid},
   title={Local Lagrangian $2$-knots are trivial},
   journal={Ann. of Math. (2)},
   volume={144},
   date={1996},
   number={1},
   pages={61--76}
}

\bib{eli-pol1}{article}{
title={The problem of Lagrangian knots in four-manifolds}
author={Eliashberg, Yakov}
author={Polterovich, Leonid}
booktitle={Geometric Topology (Athens, GA, 1993) AMS/IP Stud. Adv. Math. Amer. Math. Soc.}
date={1997}
pages={313--327}}



\bib{evans}{article}{
   author={Evans, Jonathan David},
   title={Lagrangian spheres in del Pezzo surfaces},
   journal={J. Topol.},
   volume={3},
   date={2010},
   number={1},
   pages={181--227}
}

\bib{ev-k}{article}{
title={Remarks on monotone Lagrangians in $\mathbb{C}^n$}
author={Evans, Jonathan David}
author={K\c{e}dra, Jarek}
journal={Math. Res. Lett.}
volume={21}
number={6}
date={2014}
pages={1241--1255}}

\bib{evans-pde}{book}{
   author={Evans, Lawrence C.},
   title={Partial differential equations},
   series={Graduate Studies in Mathematics},
   volume={19},
   edition={2},
   publisher={American Mathematical Society, Providence, RI},
   date={2010},
   pages={xxii+749}
}

\bib{fintushel-stern}{article}{
   author={Fintushel, Ronald},
   author={Stern, Ronald J.},
   title={Invariants for Lagrangian tori},
   journal={Geom. Topol.},
   volume={8},
   date={2004},
   pages={947--968}
}
\bib{floer}{article}{
   author={Floer, Andreas},
   title={Morse theory for Lagrangian intersections},
   journal={J. Differential Geom.},
   volume={28},
   date={1988},
   number={3},
   pages={513--547}}

\bib{frau-ziem}{article}{
title={Gromov compactness for holomorphic discs with totally real boundary conditions}
author={Frauenfelder, Urs}
author={Zehmisch, Kai}
journal={J. Fixed Point Theory Appl.}
volume={17}
number={3}
date={2015}
pages={521--540}}

\bib{giroux}{article}{
   author={Giroux, Emmanuel},
   title={Une structure de contact, m\^{e}me tendue, est plus ou moins tordue},
   language={French, with English summary},
   journal={Ann. Sci. \'{E}cole Norm. Sup. (4)},
   volume={27},
   date={1994},
   number={6},
   pages={697--705}
}

\bib{gromov}{article}{
   author={Gromov, Mikhail},
   title={Pseudo holomorphic curves in symplectic manifolds},
   journal={Invent. Math.},
   volume={82},
   date={1985},
   number={2},
   pages={307--347}
}

\bib{hatcher-wagoner}{book}{
   author={Hatcher, Allen},
   author={Wagoner, John},
   title={Pseudo-isotopies of compact manifolds},
   note={With English and French prefaces;
   Ast\'{e}risque, No. 6},
   publisher={Soci\'{e}t\'{e} Math\'{e}matique de France, Paris},
   date={1973},
   pages={i+275}
}

\bib{hoferweinstein}{article}{
title={Pseudoholomorphic curves in symplectizations with applications to the Weinstein conjecture in dimension three}
author={Hofer, Helmut}
journal={Invent. Math.}
volume={114}
number={3}
date={1993}
pages={515--563}}

\bib{hind}{article}{
title={ Lagrangian spheres in $S^2 \times S^2$}
author={Hind, Richard}
journal={Geom. Funct. Anal.}
volume={14}
number={2}
date={2004}
pages={303--318}}


\bib{hindandlisi}{article}{
title={Symplectic embeddings of polydisks}
author={Hind, Richard}
author={Lisi, Samuel}
journal={Selecta Math. (N.S.)}
volume={21}
number={3}
date={2015}
pages={1099--1120}}


\bib{hirsch}{book}{
   author={Hirsch, Morris W.},
   title={Differential topology},
   series={Graduate Texts in Mathematics},
   volume={33},
   note={Corrected reprint of the 1976 original},
   publisher={Springer-Verlag, New York},
   date={1994},
   pages={x+222},
}

\bib{lalonde-mcduff}{article}{
   author={Lalonde, Fran\c{c}ois},
   author={McDuff, Dusa},
   title={$J$-curves and the classification of rational and ruled symplectic
   $4$-manifolds},
   conference={
      title={Contact and symplectic geometry},
      address={Cambridge},
      date={1994},
   },
   book={
      series={Publ. Newton Inst.},
      volume={8},
      publisher={Cambridge Univ. Press, Cambridge},
   },
   date={1996},
   pages={3--42}
}

\bib{laudenbach}{article}{
   author={Laudenbach, Fran\c{c}ois},
   title={Submersions sur le cercle},
   journal={Bull. Soc. Math. France},
   volume={104},
   date={1976},
   number={4},
   pages={417--431}
}
\bib{laudenbach-blank}{article}{
   author={Laudenbach, Fran\c{c}ois},
   author={Blank, Samuel},
   title={Isotopie de formes ferm\'{e}es en dimension trois},
   language={French},
   journal={Invent. Math.},
   volume={54},
   date={1979},
   number={2},
   pages={103--177}
}

\bib{lau-sik}{article}{
   author={Laudenbach, Fran\c{c}ois},
   author={Sikorav, Jean-Claude},
   title={Persistance d'intersection avec la section nulle au cours d'une
   isotopie hamiltonienne dans un fibr\'{e} cotangent},
   language={French},
   journal={Invent. Math.},
   volume={82},
   date={1985},
   number={2},
   pages={349--357}}


\bib{mak-smith}{article}{
title={Non-displaceable Lagrangian links in four-manifolds}
author={Mak, Cheuk Yu},
author={Smith, Ivan},
eprint={arXiv:1909.09924 [math.SG]},
date={2019}}
%87 pages

\bib{mcduff-jams}{article}{
   author={McDuff, Dusa},
   title={The structure of rational and ruled symplectic $4$-manifolds},
   journal={J. Amer. Math. Soc.},
   volume={3},
   date={1990},
   number={3},
   pages={679--712}
}

\bib{mcduff-sal-intro}{book}{
title={Introduction to symplectic topology. Third Edition}
author={McDuff, Dusa}
author={Salamon, Dietmar}
publisher={Oxford University Press}
series={Oxford Graduate Texts in Mathematics}
city={Oxford}
date={2017}}


\bib{mcduff-sal-jcurves}{book}{
   author={McDuff, Dusa},
   author={Salamon, Dietmar},
   title={$J$-holomorphic curves and symplectic topology},
   series={American Mathematical Society Colloquium Publications},
   volume={52},
   edition={2},
   publisher={American Mathematical Society, Providence, RI},
   date={2012},
   pages={xiv+726},
}

\bib{paternain}{book}{
   author={Paternain, Gabriel P.},
   title={Geodesic flows},
   series={Progress in Mathematics},
   volume={180},
   publisher={Birkh\"{a}user Boston, Inc., Boston, MA},
   date={1999},
   pages={xiv+149}
}

\bib{polt-book}{book}{
   author={Polterovich, Leonid},
   title={The geometry of the group of symplectic diffeomorphisms},
   series={Lectures in Mathematics ETH Z\"urich},
   publisher={Birkh\"auser Verlag, Basel},
   date={2001},
   pages={xii+132},
   isbn={3-7643-6432-7}}

\bib{polterovich}{article}{
   author={Polterovich, Leonid},
   title={The Maslov class of the Lagrange surfaces and Gromov's
   pseudo-holomorphic curves},
   journal={Trans. Amer. Math. Soc.},
   volume={325},
   date={1991},
   number={1},
   pages={241--248},
}


\bib{sauvaget}{article}{
   author={Sauvaget, Denis},
   title={Curiosit\'es lagrangiennes en dimension 4},
   language={French},
   journal={Ann. Inst. Fourier (Grenoble)},
   volume={54},
   date={2004},
   number={6},
   pages={1997--2020 (2005)}
}

\bib{siebert-tian}{article}{
   author={Siebert, Bernd},
   author={Tian, Gang},
   title={On the holomorphicity of genus two Lefschetz fibrations},
   journal={Ann. of Math. (2)},
   volume={161},
   date={2005},
   number={2},
   pages={959--1020}
}

\bib{siefring}{article}{
title={Intersection theory of punctured pseudoholomorphic curves}
author={Siefring, Richard}
journal={Geom. Topol.}
volume={4}
date={2011}
pages={2351--2457}}

\bib{siefringwendl}{article}{
title={Pseudoholomorphic curves, intersections, and Morse-Bott asymptotics}
author={Siefring, Richard}
author={Wendl, Chris}
journal={In preparation}}



\bib{sikorav}{article}{
   author={Sikorav, Jean-Claude},
   title={Some properties of holomorphic curves in almost complex manifolds},
   conference={
      title={Holomorphic curves in symplectic geometry},
   },
   book={
      series={Progr. Math.},
      volume={117},
      publisher={Birkh\"{a}user, Basel},
   },
   date={1994},
   pages={165--189},
}

\bib{sikorav2}{article}{
   author={Sikorav, Jean-Claude},
   title={Formes diff\'{e}rentielles ferm\'{e}es non singuli\`eres sur le $n$-tore},
   language={French},
   journal={Comment. Math. Helv.},
   volume={57},
   date={1982},
   number={1},
   pages={79--106}
}

\bib{sullivan}{article}{
   author={Sullivan, M. G.},
   title={$K$-theoretic invariants for Floer homology},
   journal={Geom. Funct. Anal.},
   volume={12},
   date={2002},
   number={4},
   pages={810--872}
}


\bib{tillmann}{article}{
title={Tropical varieties associated to ideal triangulations: The Whitehead link complement}
author={Tillmann, Stephan},
eprint={arXiv:1911.04619 [math.GT]},
date={2019}}
%87 pages


\bib{vianna}{article}{
title={On exotic Lagrangian tori in $\mathbb{CP}^2$}
author={Vianna, Renato}
journal={Geom. Topol.}
volume={18}
number={4}
date={2014}
pages={2419--2476}}

\bib{vianna2}{article}{
   author={Vianna, Renato},
   title={Infinitely many monotone Lagrangian tori in del Pezzo surfaces},
   journal={Selecta Math. (N.S.)},
   volume={23},
   date={2017},
   number={3},
   pages={1955--1996}
}


\bib{wendlautomatic}{article}{
title={Automatic transversality and orbifolds of punctured holomorphic curves in dimension four}
author={Wendl, Chris}
journal={Comment. Math. Helv.}
volume={85}
number={2}
date={2010}
pages={347--407}}

\bib{wendlintersection}{article}{
title={Contact 3-manifolds, holomorphic curves and intersection theory}
author={Wendl, Chris}
eprint={arXiv:1706.05540 [math.SG]}
date={2017-06}}
%87 pages

\bib{wendlcurves}{book}{
   author={Wendl, Chris},
   title={Holomorphic curves in low dimensions},
   series={Lecture Notes in Mathematics},
   volume={2216},
   note={From symplectic ruled surfaces to planar contact manifolds},
   publisher={Springer, Cham},
   date={2018},
   pages={xiii+292}
}

\bib{wendlsft}{article}{
title={Lectures on Symplectic Field Theory}
author={Wendl, Chris}
eprint={arXiv:1612.01009 [math.SG]}
date={2016-12}}
%343 pages


\bib{wendlduke}{article}{
title={Strongly fillable contact manifolds and J-holomorphic foliations}
author={Wendl, Chris}
journal={Duke Math. J.}
volume={151}
number={3}
date={2010}
pages={337--384}}



%\end{biblist}
%\end{bibdiv}
%\end{document}



